Efficiently Breaking the Curse of Horizon in Off-Policy Evaluation with Double Reinforcement Learning

Off-policy evaluation (OPE) in reinforcement learning is notoriously difficult in long- and infinite-horizon settings due to diminishing overlap between behavior and target policies. In this paper, we study the role of Markovian and time-invariant structure in efficient OPE. We first derive the efficiency bounds for OPE when one assumes each of these structures. This precisely characterizes the curse of horizon: in time-variant processes, OPE is only feasible in the near-on-policy setting, where behavior and target policies are sufficiently similar. But, in time-invariant Markov decision processes, our bounds show that truly-off-policy evaluation is feasible, even with only just one dependent trajectory, and provide the limits of how well we could hope to do. We develop a new estimator based on Double Reinforcement Learning (DRL) that leverages this structure for OPE using the efficient influence function we derive. Our DRL estimator simultaneously uses estimated stationary density ratios and $q$-functions and remains efficient when both are estimated at slow, nonparametric rates and remains consistent when either is estimated consistently. We investigate these properties and the performance benefits of leveraging the problem structure for more efficient OPE.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> main_proof.tex <==

\begin{myproof}[Proof of \cref{thm:m1_bound}]
{\newedit 
We omit the proof since as it can (almost) be concluded as corollary of Theorem 1 of \citet{NathanUehara2019} where we simply set $T=\infty$ and redefine rewards by multiplying by $\gamma^t$. There are only two subtle differences. They prove the efficiency bound when $p(r_t|\cj_{a_t}),p(a_t|\cj_{s_t}),p(s_t|\cj_{r_t})$ are replaced with $p(r_t|\ch_{a_t}),p(a_t|\ch_{s_t}),p(s_t|\ch_{a_t})$, and the initial density is unknown. The former change simply means our conditioning sets are in the efficiency bound are slightly different. The latter change simply eliminates the $k=0$ term in the efficiency bound.
}
\end{myproof}

\begin{myproof}[Proof of \cref{thm:m2_bound}]
{\newedit 
Again we omit the proof as it can (almost) be concluded as a corollary of Theorem 3 of \citep{NathanUehara2019}. There is a single subtle difference. They prove the efficiency bound when the initial density is unknown. This change simply eliminates the $k=0$ term in the efficiency bound.
}

\end{myproof}

\begin{myproof}[Proof of \cref{cor:m1m2ebexist}]
We prove the statement for NMDP. For TMDP, the statement is confirmed similarly.
We have 
\begin{align*}
     &\lim_{T \to \infty }(1-\gamma)^{2}\sum_{k=1}^{T}\mathrm{E}[\gamma^{2(k-1)}\nu^{2}_{k-1} \mathrm{var}\{r_{k-1}+v(s_{k})|s_{k-1},a_{k-1}\}] \\
     &  \lnapprox \lim_{T \to \infty }(1-\gamma)^{2}\sum_{k=1}^{T}\gamma^{2(k-1)} \|\nu_k\|^{2}_{\infty}<\infty. 
\end{align*}
The final statement is clear because TMDP is included in NMDP. 
\end{myproof}


{\newedit 
\begin{myproof}[Proof of \cref{thm:m3_bound}]
Let $o=(s,a,r,s')$ and let $L_2=\{f(o):\E f^2(o)<\infty\}$.
Recall the model is 
\begin{align*}
    \cm_{3}=\{p(o)=p(s)p(a|s)p(r|s,a)p(s'|s,a) \;:\; p(s)p(a\mid s)>0\}. 
\end{align*}


\paragraph{\bf{Calculation of the tangent space}}  
We first prove that the corresponding tangent space is 
\begin{align*}
   \Tcal&=L_2\cap(\Tcal_1 +  \Tcal_2 +  \Tcal_3 + \Tcal_4), ~~\text{where}\\
   \Tcal_1 &=\braces{f(s): \E[f]=0 }\,,\Tcal_2=\braces{f(s,a): \E[f(s,a)|s]=0},\\
   \Tcal_3 &=\braces{f(s,a,s'): \E[f(s,a,s')|s,a]=0},\\
   \Tcal_4 &=\braces{f(s,a,r): \E[f(s,a,r)|s,a]=0}. 
\end{align*}
Notice that $\Tcal_j$ are orthogonal so the above sum is a direct sum.

For any submodel
\begin{align*}
    \{p_{\theta}(s)p_{\theta}(a\mid s)p_{\theta}(s'|s,a)p_{\theta}(r|s,a) \},
\end{align*}
passing through $p$ at $\theta=0$,
the score function can be decomposed as  
\begin{align*}
    g(o)
     &=g_{s}(s)+g_{a|s}(s,a)+g_{r|s,a}(s,a,r)+g_{s'|s,a}(s,a,s'),~\text{where}\\
    g_s(s) &\coloneqq \frac{d}{d\theta}\log p_{\theta}(s),\,
    g_{a|s}(s,a)\coloneqq \frac{d}{d\theta}\log p_{\theta}(a|s),\\
    g_{r|s,a}(a,s,r)&\coloneqq \frac{d}{d\theta}\log p_{\theta}(r|s,a),\,
    g_{s'|s,a}(s,a,a')\coloneqq \frac{d}{d\theta}\log p_{\theta}(s'|s,a),
\end{align*}
where these satisfy
$$
\E[g_s(s)]=0,\,
\E[g_{a|s}(s,a)\mid s]=0,\,
\E[g_{r|s,a}(s,a,r)\mid s,a]=0,\,
\E[g_{s'|s,a}(s,a,s')\mid s,a]=0.
$$
Therefore, $\Tcal$ contains the tangent space.

Next, consider any $g(o)\in\Tcal$. Since $g$ is in the direct sum $\Tcal_j$ we can write $g(o)=g_{s}(s)+g_{a|s}(s,a)+g_{r|s,a}(s,a,r)+g_{s'|s,a}(s,a,s')$. 
Let $k(x)=2(1+e^{-2x})^{-1}$. Notice that $k$ is bounded by $2$ and $k(0)=k'(0)=1$.
Consider the submodel 
\begin{align*}
    p_{\theta}(s)p_{\theta}(a|s)p_{\theta}(r|s,a)p_{\theta}(s'|s,a),\quad \theta \in (-\epsilon,\epsilon)
\end{align*}
where 
\begin{align*}
    & p_{\theta}(s)=p(s)k(\theta g_s(s)),\, p_{\theta}(a|s)=p(a|s)k(\theta  g_{a|s}(s,a)), \\ &p_{\theta}(s'|s,a)=p(s'|s,a)k(\theta g_{s'|s,a}(s,a,s')),\, p_{\theta}(r|s,a)=p(r|s,a)k(\theta g_{r|s,a}(s,a,r)). 
\end{align*}
Taking the score of this submodel we see it exactly coincides with $g$, completing the argument.




\paragraph{\bf{Calculation of gradient}}
We show the statement in two steps: (1) calculating some gradient, (2) showing this gradient is in the tangent space of $\cm_3$. Then, we can conclude that this gradient is actually the EIF. 

To calculate a gradient of the target functional $J(\epol)$ wrt the model ($\cm_3$) %
we seek $\phi$ satisfying 
\begin{align*}
   \nabla_{\theta}\rho^{\epol}(\theta)|_{\theta=0}&=\rE_{p_{b}}[\phi(s,a,r,s')g(s,a,r,s')]|_{\theta=0},\\
\rho^{\epol}(\theta) & = \lim_{T\to \infty}\rE[c_{T}(\gamma)\sum_{t=0}^{T}\gamma^{t}r_t|s_0 \sim p_{e}(s_0),a_0 \sim \epol(a_1|s_1),s_1\sim p_{\theta}(s_1|s_0,a_0),r_1\sim p_{\theta}(r_1|s_1,a_1),\cdots ], 
\end{align*}
where $p_{\theta}(s)p_{\theta}(a\mid s)p_{\theta}(s'|s,a)p_{\theta}(r|s,a)$ is any submodel, whose score function belongs to the tangent set $\Tcal$. 
Note
\begin{align*}
 \rho^{\epol}(\theta)%
  &=\lim_{T\to \infty} c_{T}(\gamma)\sum_{t=0}^T \int \gamma^{t} r_tp_{\theta}(r_t|s_t,a_t)\left\{\prod_{k=0}^t \epol(a_k|s_k)p_{\theta}(s_{k+1}|s_k,a_k)\right\}p^{(0)}_{\epol}(s_0)\mathrm{d}\lambda(\cj_{s_{t+1}})\\
  &=\int \int  c_{t}(\gamma)\gamma^{t} r_t p_{\theta}(r_t|s_t,a_t)\left\{\prod_{k=0}^t \epol(a_k|s_k)p_{\theta}(s_{k+1}|s_k,a_k)\right\}p^{(0)}_{\epol}(s_0)\mathrm{d}\lambda(\cj_{s_{t+1}})\mathrm{d}\mu'(t)  
\end{align*}
where $\mu'$ is a counting measure on $\mathbb{Z}$. This is only to emphasize that $\lim_{T\to\infty}\sum_{t=0}^{T}$ is an integral wrt the counting measure. 

Then, we have 
\begin{align} \label{eq:exchange}
      \nabla_{\theta} \rho^{\epol}(\theta)|_{\theta=0}&=C(\theta)|_{\theta=0},\\
      C(\theta)&=\lim_{T\to \infty}c_{T}(\gamma)\sum_{t=0}^{T}\int \gamma^{t} r_t \nabla p_{\theta}(r_t|s_t,a_t)\braces{\prod_{k=0}^t \epol(a_k|s_k)p_{\theta}(s_{k+1}|s_k,a_k)}p^{(0)}_{\epol}(s_0)\mathrm{d}\lambda(\cj_{s_{t+1}})  \nonumber \\
        &+\lim_{T\to \infty}c_{T}(\gamma)\sum_{t=0}^{T}\int \gamma^{t} r_tp_{\theta}(r_t|s_t,a_t) \braces{\prod_{k=0}^t \epol(a_k|s_k)\nabla p_{\theta}(s_{k+1}|s_k,a_k)}p^{(0)}_{\epol}(s_0)\mathrm{d}\lambda(\cj_{s_{t+1}}).   \nonumber
\end{align}

This exchange of integration and differentiation is justified by showing
\begin{align}\label{eq:check1}
     &\lim_{T\to \infty}c_{T}(\gamma)\sum_{t=0}^{T}\int \gamma^{t} r_t |\nabla p_{\theta}(r_t|s_t,a_t)|\braces{\prod_{k=0}^t \epol(a_k|s_k)p_{\theta}(s_{k+1}|s_k,a_k)}p^{(0)}_{\epol}(s_0)\mathrm{d}\lambda(\cj_{s_{t+1}})\\
        &+\lim_{T\to \infty}c_{T}(\gamma)\sum_{t=0}^{T}\int \gamma^{t} r_tp_{\theta}(r_t|s_t,a_t) \braces{\prod_{k=0}^t \epol(a_k|s_k)|\nabla p_{\theta}(s_{k+1}|s_k,a_k)|}p^{(0)}_{\epol}(s_0)\mathrm{d}\lambda(\cj_{s_{t+1}}). \label{eq:check2}
\end{align}
is uniformly upper-bounded by some value around some neighborhood of $\theta=0$. The first term \eqref{eq:check1} is equal to 
\begin{align*}
    &\lim_{T\to \infty}\int c_{T}(\gamma)\sum_{t=1}^{T} \rE_{\epol,\theta}[\gamma^{t} r_t |g_{R|S,A}(r_t|s_t,a_t)|]=\rE_{p^{(\infty)}_{e,\gamma}(s:\theta)\epol(a|s)p_{\theta}(r|s,a) }[r |g_{R|S,A}(r|s,a:\theta)|] \tag{Fubini}\\
    &\leq R_{\max}\rE_{p^{(\infty)}_{e,\gamma}(s:\theta)\epol(a|s) }[\rE_{p_{\theta}(r|s,a)}[|g_{R|S,A}(r|s,a:\theta)|\mid s,a]]\\
        &\leq R_{\max}\rE_{p^{(\infty)}_{e,\gamma}(s:\theta)\epol(a|s) }[\int h(r|s,a)\mathrm{d}\mu(r)]<\infty, 
\end{align*}
where $h(r|s,a)$ is some integrable function. Here we leveraged condition (d) in the definition of a one-dimensional submodel. 

The second term \eqref{eq:check2} is equal to 
\begin{align*}
     &\lim_{T\to \infty}\gamma \int c_{T}(\gamma)\sum_{c=1}^{T}\gamma^c \sum_{t=c+1}^{T}\rE_{\epol,\theta}[\gamma^{t-c-2}r_t |g_{S'|S,A}(s_{t+1}|s_t,a_t:\theta)| ]\\
     &=\gamma \rE_{p^{(\infty)}_{e,\gamma}(s:\theta)\epol(a|s)p_{\theta}(s'|s,a) }[v(s')|g_{S'|S,A}(s'|s,a:\theta)|] \tag{Fubini}\\ 
     &\leq (1-\gamma)^{-1}R_{\max}\gamma \rE_{p^{(\infty)}_{e,\gamma}(s:\theta)\epol(a|s)}[\rE_{p_{\theta}(s'|s,a)}[|g_{S'|S,A}(s'|s,a:\theta)|]] \\
      &\leq (1-\gamma)^{-1}R_{\max}\gamma \rE_{p^{(\infty)}_{e,\gamma}(s:\theta)\epol(a|s)}[\int h(s'|s,a)\mathrm{d}(s')]<\infty, 
\end{align*}
where $h(s'|s,a)$ is some integrable function. 
Combing all together, the exchange of integration and differentiation \eqref{eq:exchange} is justified. 

To derive the influence function, we continue the calculation: 
\begin{align*}
     \nabla\rho^{\epol}(\theta)|_{\theta=0}&= \rE_{p^{(\infty)}_{e,\gamma}}[r g_{R|S,A}(r|s,a)]+\gamma \rE_{p^{(\infty)}_{e,\gamma}}[v(s')g_{S'|S,A}(s'|s,a)]\\ 
     &=\rE_{p^{(\infty)}_{e,\gamma}}[\{r-\rE[r|s,a]\}g_{R|S,A}(r|s,a)]+\gamma \rE_{p^{(\infty)}_{e,\gamma}}[\{v(s')-\rE_{p^{(\infty)}_{e,\gamma}}[v(s')|s,a]\}g_{S'|S,A}(s'|s,a)]\\
     &= \rE_{p^{(\infty)}_{e,\gamma}}\left[\left\{r-\rE_{p^{(\infty)}_{e,\gamma}}[r|s,a]+\gamma v(s')-\gamma \rE[v(s')|s,a]\right\} g(s,a,r,s')\right]\\ 
     &=\rE_{p^{(\infty)}_{e,\gamma}}[\{r+\gamma v(s')-q(s,a)\} g(s,a,r,s') ]\\
    &=\rE_{p_{b}(s,a,r,s')}[(w(s)\eta(s,a)\{r+\gamma v(s')-q(s,a)\})g(s,a,r,s') ]. 
\end{align*}
Therefore, the following function is a gradient, if its $L_2$-norm is finite:
\begin{align*}
   w(s)\eta(s,a)\{r+\gamma v(s')-q(s,a)\}
\end{align*}
In addition, if it exists, it belongs to $\Tcal_1+ \Tcal_2+ \Tcal_3+ \Tcal_4$ since 
\begin{align*}
   &  w(s)\eta(s,a)\{r-\rE[r|s,a]\}\in \Tcal_4,\, w(s)\eta(s,a)\{v(s')-\rE[v(s')|s,a]\}\in \Tcal_3,\\
    &  w(s)\eta(s,a)\{r+\gamma v(s')-q(s,a)\}= w(s)\eta(s,a)\{ r-\rE[r|s,a\}+\gamma\{v(s')-\rE[v(s')|s,a]\}\}. 
\end{align*}
Thus, it is the EIF. The efficiency bound is therefore
\begin{align*}
   \rE_{p_{b}}[ w^2(s)\eta^2(a,s)\{r+\gamma v(s')-q(s,a)\}^2]. 
\end{align*}

Finally, we show that the EIF is still the same under $\cm_{3bs},\cm_{3b}$. First, the above EIF under $\cm_3$ is still a gradient under $\cm_{3bs},\cm_{3b}$.  Again, what we have to prove is that this function belongs to the tangent space. This is obvious since the tangent space of $\cm_{3b}$ is 
\begin{align*}
    L_2\cap(\Tcal_1 + \Tcal_3 +   \Tcal_4),
\end{align*}
the tangent space of $\cm_{3bs}$ is 
\begin{align*}
      L_2\cap(\Tcal_3 + \Tcal_4),
\end{align*}
and the gradient above belongs to  $L_2\cap(\Tcal_3 + \Tcal_4)\subseteq L_2\cap(\Tcal_1 + \Tcal_3 +   \Tcal_4)\subseteq L_2\cap(\Tcal_1 + \Tcal_2 + \Tcal_3 +   \Tcal_4)$. 
\end{myproof}
}



{\newedit 
\begin{myproof}[Proof of \cref{thm:m1_inf}]

In this proof, we write $q^{\omega_N}_k$ as $q_k$ to simplify the notation. Define:
\begin{align*}
\psi(\{\hat{\nu}_{k}\},\{\hat{q}_k\})=
    \sum_{k=0}^{\omega_N}\hat{\nu}_{k}r_k-\{\hat{\nu}_{k-1} \hat{q}_k-\hat{\nu}_{k}\rE_{\epol}[\hat{q}_k(s_k,a_k)|s_k]\}. 
\end{align*}
The estimator $\hat{\rho}^{\cm1}_{\mathrm{DRL}(\cm_1)}$ is then given by
\begin{align*}
\frac{N_0}{N}\P_{\dm_0}\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})+\frac{N_1}{N}\P_{\dm_1}\psi(\{\hat{\nu}^{[0]}_{k}\},\{\hat{q}^{[0]}_k\}),
\end{align*}
where $\P_{\dm_j}$ is the empirical average over $\dm_j$ and $N_j$ is the sample size of each.
Then, we have 
\begin{align}
    \sqrt{N}(\P_{\dm_0}\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\rho^{\epol}_{\omega_N})&= \sqrt{N/N_0}\bG_{N_0}[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{q_k\})]
    \label{eq:term1_drl}
    \\
    &+\sqrt{N/N_0}\bG_{N_0}[\psi(\{\nu_{k}\},\{q_k\}) ] 
       \label{eq:term1_dr2}
    \\
    &+\sqrt{N}(\rE[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})|\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{(1)}_k\} ]-\rho^{\epol}_{\omega_N} ).    \label{eq:term1_dr3}
\end{align}
We analyze each term. To do that, we use the following relation:
\begin{align*}
&\psi(\{\hat{\nu}_{k}\},\{\hat{q}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})=D_1+D_2+D_3,\quad\text{where}\\
&D_1 =\sum_{k=0}^{w_N}(\hat{\nu}_{k}-\nu_{k})(-\hat{q}_k+q_k)+(\hat{\nu}_{k-1}-\nu_{k-1})(-\hat{v}_k+v_k), \\
&D_2 =\sum_{k=0}^{\omega_N}\nu_{k}(\hat{q}_k-q_k)+\nu_{k-1}(\hat{v}_k-v_k), \\
&D_3 =\sum_{k=0}^{\omega_N}(\hat{\nu}_{k}-\nu_{k} )(r_k-q_k+v_{k+1}).
\end{align*}

First, we show the term \eqref{eq:term1_drl} is $\smallo_{p}(1)$. 

\paragraph*{\bf{The term \eqref{eq:term1_drl} is $\smallo_{p}(1)$.}}

If we can show that for any $\epsilon>0$, 
\begin{align}
\label{eq:process_m1}
\lim_{n\to \infty}\sqrt{N_0}P[&\P_{\dm_0}[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})]\\&\notag- 
 \rE[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})|\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\} ]>\epsilon|\mathcal{D}_1]=0, %
\end{align}
Then, by bounded convergence theorem, we would have 
\begin{align*}
  \lim_{n\to \infty}\sqrt{N_0}P[&\P_{\dm_0}[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-
  \psi(\{\nu_{k}\},\{{q}_k\})]\\&-\rE[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})|\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\}]>\epsilon]=0,
\end{align*}
yielding the statement. 

To show \eqref{eq:process_m1}, we show that the conditional mean is $0$ and conditional variance is $\smallo_p(1)$. 
The conditional mean is 
\begin{align*}
&\rE[\P_{\dm_0}[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})]\\&\qquad\qquad\qquad\qquad\qquad-\rE[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})\mid \{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\}]|\mathcal{D}_1] \\
&=0.
\end{align*}
Here, we leverage the sample splitting construction, that is, $\hat{\nu}^{[1]}_{k}$ and $\hat{q}^{[1]}_{k}$ only depend on $\mathcal{D}_1$. The conditional variance is 
\begin{align*}
&\mathrm{var}[\sqrt{N_0}\P_{\dm_0}[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})]|\mathcal{D}_1]\\
&\qquad\qquad= \rE[D^{2}_1+D^{2}_2+D^{2}_3+2D_{1}D_{2}+2D_{2}D_{3}+2D_{2}D_{3} \mid \mathcal{D}_1] \\ 
&\qquad\qquad=\omega^{2}_N \max\{\Op((\kappa^\nu_N)^2),\Op((\kappa^q_N)^2),\Op(\kappa^\nu_N\kappa^q_N)\}=\smallo_p(1).
\end{align*}
Here, we used the convergence rate assumptions (\ref{thm:m1_inf}c) and the relation $\|\hat{v}^{[1]}_{k}-v_{k}\|_{2}\leq C\|\hat{q}^{[1]}_{k}-q_{k}\|_{2}$ arising from the fact that the former is the marginalization of the latter over $\pi_{e,k}$ and Jensen's inequality. Then, from Chebyshev's inequality:
\begin{align*}
&\sqrt{N_0}P[\P_{\dm_0}[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})]-\rE[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})|\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\} ]>\epsilon|\mathcal{D}_1] \\
&\leq \frac{1}{\epsilon^{2}}\mathrm{var}[\sqrt{N_0}\P_{\dm_0}[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\psi(\{\nu_{k}\},\{{q}_k\})]|\mathcal{D}_1]=\smallo_{p}(1).\qedhere
\end{align*}


\paragraph*{ \bf{The term \cref{eq:term1_dr3} is $\smallo_{p}(1)$.}}

\begin{align*}
&\sqrt{N}\rE[\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\rE[\psi(\{\nu_{k}\},\{{q}_k\})]|\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\}]\\ 
&=\sqrt{N}\rE[\sum_{k=0}^{\omega_N}(\hat{\nu}^{[1]}_{k}-\nu_{k} )(-\hat{q}^{[1]}_k+q_k)+(\hat{\nu}^{[1]}_{k-1}-\nu_{k-1})(-\hat{v}_k+v_k)|\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\}]\\
    &+\sqrt{N}\rE[\sum_{k=0}^{\omega_N}\nu_{k}(\hat{q}^{[1]}_k-q_k)+\nu_{k-1}(\hat{v}_k-v_k)|\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\}] \\
    &+\sqrt{N}\rE[\sum_{k=0}^{\omega_N}(\hat{\nu}^{[1]}_{k}-\nu_{k} )(r_k-q_k+v_{k+1})|\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\}] \\
&=\sqrt{N}\rE[\sum_{k=0}^{\omega_N}(\hat{\nu}^{[1]}_{k}-\nu_{k} )(-\hat{q}^{[1]}_k+q_k)+(\hat{\nu}^{[1]}_{k-1}-\nu_{k-1})(-\hat{v}_k+v_k)|\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\}] \\
&= \sqrt{N}\sum_{k=0}^{\omega_N} \mathcal{O}(\|\hat{\nu}^{[1]}_{k}-\nu_{k}\|_{2}\|\hat{q}^{[1]}_{k}-q_{k}\|_{2}) =\sqrt{N}\sum_{k=0}^{\omega_N}\kappa^\nu_N \kappa^q_N=\smallo_{p}(1).  %
\end{align*}
Here, we have used the assumption (\ref{thm:m1_inf}e). 

\paragraph*{\bf{Combining all things}}

Finally, we get 
\begin{align*}
    \sqrt{N}(\P_{\dm_0}\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\rho^{\epol}_{\omega_N})=\sqrt{N/N_0}\bG_{\dm_0}[\psi(\{\nu_{k}\},\{q_k\}) ]+\smallo_{p}(1).
\end{align*}
By flipping the role, 
\begin{align*}
   \sqrt{N}(\P_{\dm_1}\psi(\{\hat{\nu}^{[0])}_{k}\},\{\hat{q}^{[0])}_k\})-\rho^{\epol}_{\omega_N})=\sqrt{N/N_1}\bG_{\dm_1}[\psi(\{\nu_{k}\},\{q_k\}) ]+\smallo_{p}(1).
\end{align*}
Therefore, 
\begin{align*}
    &\sqrt{N}(\hat{\rho}_{\mathrm{DRL(\cm_1)}}-\rho^{\epol}_{\omega_N})\\
    &=  N_0/N\times \sqrt{N}\psi(\{\hat{\nu}^{[1]}_{k}\},\{\hat{q}^{[1]}_k\})-\rho^{\epol}_{\omega_N})+ N_1/N\times \sqrt{N}(\P_{\dm_1}\psi(\{\hat{\nu}^{[0]}_{k}\},\{\hat{q}^{[0]}_k\})-\rho^{\epol}_{\omega_N}) \\
    &=\sqrt{N_0/N}\bG_{N_0}[\psi(\{\nu_{k}\},\{q_k\})  ]+\sqrt{N_1/N}\bG_{N_1}[\psi(\{\nu_{k}\},\{q_k\}) ]+\smallo_{p}(1)\\
    &=\bG_{N}[\psi(\{\nu_{k}\},\{q_k\}) ] +\smallo_{p}(1).
\end{align*}
Finally, from the assumption (\ref{thm:m1_inf}a),(\ref{thm:m1_inf}b)(\ref{thm:m1_inf}d) and CLT, the efficiency is concluded. This estimator is also regular from \cref{thm:gradients}. 


\end{myproof}
}

\begin{myproof}[Proof of \cref{thm:m2_inf}]
The proof is similar to that of \cref{thm:m1_inf}
\end{myproof}



{\newedit 
\begin{myproof}[Proof of \cref{thm:m3_inf,thm:m3_inf_adaptive}]
First, We provide the proof the cross-fitting version. Then, we provide the proof of the adaptive version. 

In the cross-fitting version, the estimator is given by 
\begin{align*}
\frac{n_0}{n}\P_{\Dcal_0}\psi(\hat w^{[1]},\hat q^{[1]})+\frac{n_1}{n}\P_{\Dcal_1}\psi(\hat w^{[0]},\hat q^{[0]}) 
\end{align*}
where $\P_{\Dcal_0}$ is a sample average over a set of samples in one fold, and  $\P_{\Dcal_1}$ is a sample average over a set of samples in another fold. Then, we have 
\begin{align}
    \sqrt{n}(\P_{\dm_0}\psi(\hat w^{[1]},\hat q^{[1]})-\rho^{\epol})&= \sqrt{n/n_0}\bG_{n_0}[\psi(\hat w^{[1]},\hat q^{[1]})-\psi(w^{[1]}, q^{[1]})]
    \label{eq:term3_drl}
    \\
    &+\sqrt{n/n_0}\bG_{n_0}[\psi(w^{[1]}, q^{[1]})] 
       \label{eq:term3_dr2}
    \\
    &+\sqrt{n}(\rE[\psi(\hat w^{[1]},\hat q^{[1]})\mid \hat w^{[1]},\hat q^{[1]} ]-\rho^{\epol} ).    \label{eq:term3_dr3}
\end{align}

We analyze each term. Here, we have 
\begin{align*}
\psi(\hat{w},\hat{q})-\psi(w,q)&=D_1+D_2+D_3, \\
  D_1 & =\{\hat{w}(s)-w(s)\}\eta(s,a)\{r-q(s,a)+\gamma v(s')\}, \\
D_2 &= w(s)\eta(s,a)\{q(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v(s')\}+(1-\gamma)\rE_{p^{(0)}_{\epol}}[v'(s)-v(s)], \\
 D_3 &=\{\hat{w}(s)-w(s)\}\eta(s,a)\{q(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v(s')\}.
\end{align*}

\paragraph{\bf{Term \eqref{eq:term3_drl} is $\op(1)$ }}

We show that the conditional variance given $\Dcal_1$ is  $\op(1)$. The rest of the argument is the same as the proof of \cref{thm:m1_inf}. 
The conditional variance is 
\begin{align*}
    \var[\sqrt{n_0}\P_{\Dcal_0}[ \psi(\hat{w},\hat{q})-\psi(w,q)    ]|\Dcal_1 ]&\leq \E[D^2_1+D^2_2+D^3_2+2D_1D_2+2D_2D_3+2D_1D_3 |\Dcal_1 ] \\ 
    &=\op(1). 
\end{align*}
Here, we use 
\begin{align*}
     \|\hat v(s')-v(s')\|_2 \leq \sqrt{C_{S'}}\|\hat q(s,a)-q(s,a)\|_2. 
\end{align*}
from Jensen's inequality. 

\paragraph{\bf{Term \eqref{eq:term3_dr3} is $\op(1)$ }}

\begin{align*}
   | \E[D_1+D_2+D_3|\Dcal_1]|&\leq \|\hat w-w\|_2\|\eta\|_2\|\hat q-q\|_2+ \|\hat w-w\|_2\|\eta\|_2\|\hat v(s')-v(s)\|_2 \\ 
   &\leq \|\hat w-w\|_2\|\eta\|_2\|\hat q-q\|_2+\sqrt{\gamma C_S'} \|\hat w-w\|_2\|\eta\|_2\|\hat q-q\|_2 \\ 
   &=\kappa^w_n\kappa^q_n=\op(n^{-1/2}). 
\end{align*}


\paragraph{\bf{Proving efficiency} }

\begin{align*}
    &\sqrt{n}(\P_{\dm_0}\psi(\hat w^{[1]},\hat q^{[1]})+\P_{\dm_1}\psi(\hat w^{[0]},\hat q^{[0]})-\rho^{\epol})\\
    &=\sqrt{n/n_0}\bG_{n_0}[\psi(w^{}, q^{})]+ \sqrt{n/n_1}\bG_{n_1}[\psi(w^{}, q^{})]+\op(n^{-1/2})\\
    &=\bG_{n}[\psi(w^{}, q^{})] +\op(n^{-1/2}). 
\end{align*}
Finally, from CLT, the final statement is concluded. 

{\newedit 
\paragraph*{\bf{Proof of adaptive version}}

The adaptive version is similarly proved. 
\begin{align}
    \sqrt{n}(\P_{n}\psi(\hat w^{[1]},\hat q^{[1]})-\rho^{\epol})&=\bG_{n}[\psi(\hat w^{[1]},\hat q^{[1]})-\psi(w^{[1]}, q^{[1]})]
    \label{eq:term3_drl_ada}
    \\
    &+\bG_{n}[\psi(w^{[1]}, q^{[1]})] 
       \label{eq:term3_dr2_ada}
    \\
    &+\sqrt{n}(\rE[\psi(\hat w^{[1]},\hat q^{[1]})\mid \hat w^{[1]},\hat q^{[1]} ]-\rho^{\epol} ).    \label{eq:term3_dr3_ada}
\end{align}
The third term is $\op(1)$ following the similar logic as before. We prove the first term is $\op(1)$. From \citet[Lemma 19.24]{VaartA.W.vander1998As}, what we need to prove is 
\begin{align*}
    \mathbb{F}=\{\psi(w,q):w\in \Fcal_{w}, q\in \Fcal_q\}
\end{align*}
belongs to a Donsker class. If we can prove the uniform entropy integral:
\begin{align*}
    \int_{0}^1 \sqrt{\log \sup_{U}\mathcal{N}(\tau, \mathbb{F},L_2(U))}d(\tau), 
\end{align*}
is finite, from \citet[Theorem 19.14]{VaartA.W.vander1998As}, the class $\mathbb{F}$ belongs to a Donsker class. Here, 
\begin{align*}
    \log \sup_{U}\mathcal{N}(\tau, \mathbb{F},L_2(U)) & \leq    \log \sup_{U}\mathcal{N}(\tau, \mathbb{F},L_{2}(U))\\
    &\leq C \{\log \mathcal{N}(\tau,\Fcal_{w},L_{\infty}(U))+\log \sup_{U}\mathcal{N}(\tau, \Fcal_q,L_{\infty}(\cdot)) \} \\ 
    &\leq C (1/\tau)^{\beta}< C (1/\tau)^{2}.  
\end{align*}
From the second line to the third line, we use \citet[Leemma 9]{UeharaMasatoshi2021FSAo}. Thus, the uniform entropy integral is finite, which leads to the conclusion that first term \eqref{eq:term3_drl_ada} is $\op(1)$.
}

\end{myproof}
}


{\blockedit 
\begin{myproof}[Proof of \cref{thm:db_m3}]
We provide the proof the cross-fitting version. The estimator is given by 
\begin{align*}
\frac{n_0}{n}\P_{\Dcal_0}\psi(\hat w^{[1]},\hat q^{[1]})+\frac{n_1}{n}\P_{\Dcal_1}\psi(\hat w^{[0]},\hat q^{[0]}) 
\end{align*}
where $\P_{\Dcal_0}$ is a sample average over a set of samples in one fold, and  $\P_{\Dcal_1}$ is a sample average over a set of samples in another fold. Then, we have 
\begin{align}
  \P_{\dm_0}\psi(\hat w^{[1]},\hat q^{[1]})&= \sqrt{1/n_0}\bG_{n_0}[\psi(\hat w^{[1]},\hat q^{[1]})-\psi(w^{\dagger}, q^{\dagger})]
    \label{eq:term3_drl_m3}
    \\
    &+\rE[\psi(\hat w^{[1]},\hat q^{[1]})\mid \hat w^{[1]},\hat q^{[1]} ]-\rE[\psi( w^{\dagger}, q^{\dagger})]   \label{eq:term3_dr3_m3} \\ 
    &+  \P_{\dm_0}\psi( w^{\dagger}, q^{\dagger}). 
\end{align}
Then, we have 
\begin{align*}
\rE[\psi(\hat{w},\hat{q})|\hat{w},\hat{q}]&=\rE[\{\hat{w}(s)-w^{\dagger}(s)\}\eta(s,a)\{r-q^{\dagger}(s,a)+\gamma v^{\dagger}(s')\}]+ \\
 &+\rE[w^{\dagger}(s)\eta(s,a)\{q^{\dagger}(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v^{\dagger}(s')\}]+(1-\gamma)\rE_{p^{(0)}_{e}}[v'(s)-v^{\dagger}(s)] \\
 &+\rE[\{\hat{w}(s)-w^{\dagger}(s)\}\eta(s,a)\{q^{\dagger}(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v^{\dagger}(s')\}] \\
 &+\rE[\{\hat{v}(s')-v^{\dagger}(s')-\hat{q}(s,a)+q^{\dagger}(s,a)\}|\hat{w},\hat{q}]\\
&+\rE[\psi(w^{\dagger},q^{\dagger})|\hat{w},\hat{q}] \\
&=\mathcal{O}(\| \hat{w}(s)-w^{\dagger}(s)\|_2,\|\hat{q}(s,a)-q^{\dagger}(s,a)\|_2,\|\hat{v}(s')-v^{\dagger}(s') \|_{2})+\rE[\psi(w^{\dagger},q^{\dagger})] \\
&=\op(1)+\rE[\psi(w^{\dagger},q^{\dagger})].
\end{align*}
Thus, the term \eqref{eq:term3_dr3_m3} is $\op(1)$. Thus, the remaining part is proving when at least one model is well-specified, the term $\P_{\dm_0}\psi( w^{\dagger}, q^{\dagger})$ is consistent. 

\paragraph*{\bf{$q$-model is well-specified .}}

Consider the case where $q^{\dagger}(s,a)=q(s,a)$;
\begin{align*}
    &\rE[\psi(w^{\dagger},q^{\dagger})]=\rE[(1-\gamma)\rE_{p^{(0)}_{e}}[v(s)]+w^{\dagger}(s)\eta(s,a)\{r+\gamma v(s')-q(s,a)\}] \\
    &= (1-\gamma)\rE_{p^{(0)}_{\epol}}[v(s)]=\rho^{\epol}. 
\end{align*}
This implies when the q-model is consistent, the estimator $\hat{\rho}_{\mathrm{DRL(\cm_3)}}$ is also consistent. 

\paragraph*{\bf{$w$-model is well-specified.}}

Consider the case where $w^{\dagger}(s)=w(s)$;
\begin{align}
    \rE[\psi(w^{\dagger},q^{\dagger})]&=\rE[(1-\gamma)\rE_{p^{(0)}_{e}}[v^{\dagger}(s)]+w(s)\eta(s,a)\{r+\gamma v^{\dagger}(s')-q^{\dagger}(s,a)\}] \nonumber\\
    &=(1-\gamma)\rE_{p^{(0)}_{e}}[v^{\dagger}(s)]+\rE[w(s)\eta(s,a)r]+\rE[w(s)\eta(s,a)\gamma v^{\dagger}(s')] \label{eq:db1}\\
    &-\rE[w(s)\eta(s,a) q^{\dagger}(s,a)] \nonumber \\ 
    &=\rE[w(s)\eta(s,a)r]+\rE[w(s) v^{\dagger}(s)]-\rE[w(s)\eta(s,a) q^{\dagger}(s,a)] \label{eq:db2}\\ 
    &=\rE[w(s)\eta(s,a)r]=\rho^{\epol}.\label{eq:db3}
\end{align}
From \eqref{eq:db1} to \eqref{eq:db2}, we use a result 
\begin{align*}
    (1-\gamma)\rE_{p^{(0)}_{\epol}}[v^{\dagger}(s)]+\rE[w(s)\eta(s,a)\gamma v^{\dagger}(s')]=\rE[w(s) v^{\dagger}(s)]
\end{align*}
from \cref{lem:ratio-estimation}. From \eqref{eq:db2} to \eqref{eq:db3}, we use a result 
\begin{align*}
    \rE[w(s)\eta(s,a) q^{\dagger}(s,a)]= \rE[w(s)\rE[\eta(s,a) q^{\dagger}(s,a)|s]]=\rE[w(s)v^{\dagger}(s)]. 
\end{align*}
This implies when the ratio model is correct, the estimator $\hat{\rho}_{\mathrm{DRL(\cm_3)}}$ is also consistent. 


\end{myproof}
}




{\blockedit 
\begin{myproof}[Proof of \cref{thm:db_n}]
We only provide the proof the cross-fitting version. The adaptive version is similarly proved. The estimator is given by 
\begin{align*}
\frac{n_0}{n}\P_{\Dcal_0}\psi(\hat w^{[1]},\hat q^{[1]})+\frac{n_1}{n}\P_{\Dcal_1}\psi(\hat w^{[0]},\hat q^{[0]}). 
\end{align*}
We have the following decomposition: 
\begin{align}
    \sqrt{n}(\P_{\Dcal_0}\psi(\hat w^{[1]},\hat q^{[1]})-\rho^{\epol}) 
    &= \sqrt{n/n_0}\{\bG_{n_0}\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\bG_{n_0}\psi(w^{\dagger},q^{\dagger})\}+ \label{eq:db13}\\
    &+\sqrt{n}(\rE[\psi(\hat{w}^{[1]},\hat{q}^{[1]})|\hat{w}^{[1]},\hat{q}^{[1]}]-\rE[\psi(w^{\dagger},q^{\dagger})]) \label{eq:db23} \\
    &+\sqrt{n}( \rE[\psi(w^{\dagger},q^{\dagger})]-\rho^{\epol}) \label{eq:db33}\\
    &+\sqrt{n/n_0}\bG_{n_0}\psi(w^{\dagger},q^{\dagger}). \nonumber
\end{align}
The term \eqref{eq:db13} is $\op(1)$ as in the proof of \cref{thm:m3_inf}. The term \eqref{eq:db23} is $\bigO_p(1)$ as in the proof of \cref{thm:db_m3}:
\begin{align*}
\rE[\psi(\hat{w}^{[1]},\hat{q}^{[1]})|\hat{w}^{[1]},\hat{q}^{[1]}]&=\mathcal{O}(\| \hat{w}^{[1]}(s)-w^{\dagger}(s)\|_2,\|\hat{q}^{[1]}(s,a)-q^{\dagger}(s,a)\|_2,\|\hat{v}^{[1]}(s')-v^{\dagger}(s') \|_{2})+\rE[\psi(w^{\dagger},q^{\dagger})] \\
&=\bigO_p(n^{-1/2})+\rE[\psi(w^{\dagger},q^{\dagger})].
\end{align*}

The term \eqref{eq:db33} is $0$ following the argument in the proof of \cref{thm:db_m3}. Then, we obtain $\sqrt{n}(\hat{\rho}_{\mathrm{DRL(\cm_3)}}-\rho^{\epol})=\bG_{n}\psi(w^{\dagger},q^{\dagger})+\bigO_p(1)=\bigO_p(1)$.
\end{myproof}
}



{\blockedit\begin{myproof}[Proof of \cref{thm:ideal_m3}]
For the ease of the notation, we assume $N=1$. The extension to general $N$ is straightforward. 

Under the assumptions, $\psi(s,a,r,s';w,q)$ is bounded.
Invoking \citet[Theorem 18.5.4]{ibragimov1975independent}, we obtain
that $\sqrt{T}\prns{\P_T[\psi(s,a,r,s';w,q)]-\rho^{\epol}}$ converges to a normal distribution with zero mean and the variance: 
\begin{align}\notag
    \mathrm{var}[\phi_\text{eff}(s_0,a_0,r_0,s_1)]+2\sum_{i=1}^{\infty}\mathrm{cov}[\phi_\text{eff}(s_0,a_0,r_0,s_1),\phi_\text{eff}(s_i,a_i,r_i,s_{i+1})], 
\end{align}
where $\phi_\text{eff}$ is as in \cref{thm:m3_bound}. The first term is $\mathrm{EB}(\cm_3)$.
The second term is zero because 
\begin{align*}
    &\rE[\phi_\text{eff}(s_0,a_0,r_0,s_1)\phi_\text{eff}(s_i,a_i,r_i,s_{i+1})] \\
    &= \rE[\phi_\text{eff}(s_0,a_0,r_0,s_1)\rE[\phi_\text{eff}(s_i,a_i,r_i,s_{i+1})\mid s_{i-1},a_{i-1},r_{i-1},s_{i}]]=0. \qedhere
\end{align*}
\end{myproof}}

{\blockedit
\begin{myproof}[Proof of \cref{thm:m3_eff_cro}]
Using the short-hand $\psi(w',q')$ for $\psi(s,a,r,s';w',q')$
and $N_j=\abs{\dm_j}$,
the estimator $\hat{\rho}_{\mathrm{DRL(\cm3)}}$ is given by 
\begin{align*}
\frac{N_0}{N}\P_{\dm_0}\P_{T}\psi(\hat{w}^{[1]},\hat{q}^{[1]})+\frac{N_1}{N}\P_{\dm_1}\P_{T}\psi(\hat{w}^{[0]},\hat{q}^{[[0]}),
\end{align*}
where $\P_{\dm_j}$ is the empirical average on the samples in $\dm_j$. 

Then, we have 
\begin{align}
    \sqrt{NT}(\P_{\dm_0}\P_{T}\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\rho^{\epol})&= \sqrt{N/N_0}\bG_{\dm_0,T}[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)]
    \label{eq:term1_dr31}
    \\
    &\phantom{=}+\sqrt{N/N_0}\bG_{\dm_0,T}[\psi(w,q)] 
      \nonumber
    \\
    &\phantom{=}+\sqrt{NT}(\rE[\psi(\hat{w}^{[1]},\hat{q}^{[1]})|\hat{w}^{[1]},\hat{q}^{[1]} ]-\rho^{\epol} )   \label{eq:term1_dr33},
\end{align}
where $\bG_{\dm_0,T}$ is an empirical process defined over the all sample in the first fold. 
Here, we have 
\begin{align*}
&\P_{T}\psi(\hat{w},\hat{q})-\P_{T}\psi(w,q) \\
&=\P_{T}[\{\hat{w}(s)-w(s)\}\eta(s,a)\{r-q(s,a)+\gamma v(s')\}] \\
 &\phantom{=}+\P_{T}[w(s)\eta(s,a)\{q(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v(s')\}]+(1-\gamma)\rE_{p^{(0)}_{\epol}}[v'(s)-v(s)] \\
 &\phantom{=}+\P_{T}[\{\hat{w}(s)-w(s)\}\eta(s,a)\{q(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v(s')\}].
\end{align*}

We analyze each term. First, we show the term \cref{eq:term1_dr31} is $\smallo_{p}(1)$. 

\paragraph*{\textbf{The term \eqref{eq:term1_dr31} is $\smallo_{p}(1)$}}


Consider the case $N_0=1$. The case with $N_0>1$ similarly holds.
If we can show that for any $\epsilon>0$, 
\begin{align}
\label{eq:process_m1_1}
\lim_{T\to \infty}\sqrt{T}P[&\P_{T}[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)]\\&\notag- 
 \rE[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)|\hat{w}^{[1]},\hat{q}^{[1]} ]>\epsilon|\mathcal{D}_1]=0, %
\end{align}
then, by bounded convergence theorem, we would have 
\begin{align*}
  \lim_{T\to \infty}\sqrt{T}P[&\P_{T}[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-
  \psi(w,q)]\\&-\rE[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)|\hat{w}^{[1]},\hat{q}^{[1]}]>\epsilon]=0,
\end{align*}
which yields the statement. 

To show \cref{eq:process_m1_1}, we show that the conditional mean is $0$ and conditional variance is $\smallo_p(1)$. 
The conditional mean is 
\begin{align*}
&\rE[\P_{T}[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)|\hat{w}^{[1]},\hat{q}^{[1]}]\\&\qquad\qquad\qquad\qquad\qquad-\P[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)]|\mathcal{D}_1]
=0.
\end{align*}
Here, we leverage the sample-splitting construction, that is, $\hat{w}^{[1]}$ and $\hat{q}^{[1]}$ only depend on $\mathcal{D}_1$, and $\mathcal{D}_1,\,\mathcal{D}_0$ are independent. The conditional variance is 
\begin{align*}
&\mathrm{var}[\sqrt{T}\P_{T}[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)]|\mathcal{D}_1]=\rE\left[T\left\{\P_{T}[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)]\right\}^2|\mathcal{D}_1\right]\\
&=\frac{1}{T}\left[\sum_{i=0}^{T} \max\{\Op((\kappa^w_N)^2),\Op((\kappa^q_N)^2)\}+2\sum_{i<j}^{T}\rho_{\|i-j\|} \max\{\Op((\kappa^w_N)^2),\Op((\kappa^q_N)^2)\}\right]\\
&=\smallo_p(1).
\end{align*}
Then, from Chebyshev's inequality:
\begin{align*}
&\sqrt{T}P[\P_{T}[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)]-\rE[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)|\hat{w}^{[1]},\hat{q}^{[1]} ]>\epsilon|\mathcal{D}_1] \\
&\leq \frac{1}{\epsilon^{2}}\mathrm{var}[\sqrt{T}\P_{T}[\psi(\hat{w}^{[1]},\hat{q}^{[1]})-\psi(w,q)]|\mathcal{D}_1]=\smallo_{p}(1).\qedhere
\end{align*}




\paragraph*{\textbf{Second Term}}
We show 
$$\sqrt{NT}(\rE[\psi(\hat{w}^{[1]},\hat{q}^{[1]})|\hat{w}^{[1]},\hat{q}^{[1]}]-\rho^{\epol})=\op(1).$$

Assume $N_0=1$ for simplicity. The case with $N_0>1$ similarly holds. Noting $\rE[(\hat{q}(s,a)-q(s,a))^{2}]\geq \rE[(\hat{v}(s')-v(s'))^{2}]$ from Jensen's inequality, we have 
\begin{align*}
&|\sqrt{T}\rE[\psi(s,a,r,s';\hat{w}^{[1]},\hat{q}^{[1]})-\psi(s,a,r,s';w,q)|\hat{w}^{[1]},\hat{q}^{[1]}] |\\
=&|\sqrt{T}\rE[(\hat{w}(s)-w(s))\eta(s,a)(r-q(s,a)+\gamma v(s'))|\hat{w}^{[1]},\hat{q}^{[1]}]+ \\
 &\sqrt{T}\rE[w(s)\eta(s,a)\{q(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v(s')\}+(1-\gamma)\rE_{p^{(0)}_{\epol}}[\hat{v}(s)-v(s)]||\hat{w},\hat{q}]+ \\
 &\sqrt{T}\rE[\{\hat{w}(s)-w(s)\}\eta(s,a)\{q(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v(s')\}|\hat{w}^{[1]},\hat{q}^{[1]}]|\\
 =&|\sqrt{T}\rE[\{\hat{w}(s)-w(s)\}\eta(s,a)\{q(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v(s')\}|\hat{w}^{[1]},\hat{q}^{[1]}]|\\
\leq & \sqrt{T}\|\hat{w}^{[1]}(s)-w(s)\|_{2}\|\eta(s,a)\|_2\|q(s,a)-\hat{q}^{[1]}(s,a)\|_{2}=\smallo_{p}(1). 
\end{align*}

\paragraph*{\textbf{Combining all results}}

Combining all result,  
\begin{align*}
    \sqrt{NT}(\hat{\rho}_{\mathrm{DRL(\cm_3)}}-\rho^{\epol})=\mathbb{G}_{N,T}\psi(w,q)+\op(1).
\end{align*}
Then, from \cref{eq:mixing relationships} and \citet[Theorem 18.5.4]{ibragimov1975independent} the statement is concluded as in \cref{thm:ideal_m3}. 
\end{myproof}
}

{\newedit
\begin{myproof}[Proof of \cref{thm:m3_eff_cro2}]
We focus on $N=1$, which is most relevant for cross-time-fitting; also $N>1$ easily follows similarly.
Using the short-hand $\psi(w',q')$ for $\psi(s,a,r,s';w',q')$ and $T_j=\abs{\ct_j}$,
the estimator $\hat{\rho}_{\mathrm{DRL}(\cm3)}$ is given by 
\begin{align*}
\frac{T_0}{T}\P_{\ct_0}\psi(\hat{w}^{[2]},\hat{q}^{[2]})+\frac{T_1}{T}\P_{\ct_1}\psi(\hat{\nu}^{[3]},\hat{q}^{[3]})+\frac{T_2}{T}\P_{\ct_2}\psi(\hat{\nu}^{[0]},\hat{q}^{[0]})+\frac{T_3}{T}\P_{\ct_3}\psi(\hat{\nu}^{[1]},\hat{q}^{[1]}),
\end{align*}
where $\P_{\ct_j}$ is the empirical average on the samples in $\ct_j$.

The proof now proceeds as in \cref{thm:m3_eff_cro}. 
In particular, we have to deal with the dependence across folds more carefully. 

First, we show the analysis of the stochastic equicontinuity term. To prove it, we must leverage the fact that $\ct_0$ and $\ct_1$ are separated by $T/4$ time steps, rather than being independent, unlike \cref{thm:m3_eff_cro}. 

\paragraph*{\textbf{First part}: $\bG_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]=\op(1)$ }
\begin{myproof}
If we can show that for any $\epsilon>0$, 
\begin{align}
\label{eq:process_m1_}
\lim_{T\to \infty}\sqrt{T_0}P[&\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]\\&\notag- 
 \rE[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)|\hat{w}^{[2]},\hat{q}^{[2]} ]>\epsilon|\mathcal{T}_2]=0, %
\end{align}
Then, by bounded convergence theorem, we would have 
\begin{align*}
  \lim_{T\to \infty}\sqrt{T_0}P[&\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-
  \psi(w,q)]\\&-\rE[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)|\hat{w}^{[2]},\hat{q}^{[2]}]>\epsilon]=0,
\end{align*}
yielding the statement. 

To show \eqref{eq:process_m1_}, we show that the conditional mean given $\mathcal{T}_2$ is $\smallo_p(1)$ and conditional variance given $\mathcal{T}_2$ is $\smallo_p(1)$. The conditional mean given $\mathcal{T}_2$ is 
\begin{align}
&|\E[\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]-\E[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]|\mathcal{T}_2]|  \nonumber  \\
&=|\E[\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]|\ct_2]-\E[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q) \mid \hat{w}^{[2]},\hat{q}^{[2]}] | \label{eq:show2} \\
&\leq |\P[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)| \mid \hat{w}^{[2]},\hat{q}^{[2]}]-\E[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q) \mid \hat{w}^{[2]},\hat{q}^{[2]}]|+\op(1) \label{eq:show3} \\
&= \smallo_p(1).\nonumber 
\end{align}

Here, we leverage the sample splitting construction, that is, $\hat{w}^{[2]}_{k}$ and $\hat{q}^{[2]}_{k}$ only depend on $\mathcal{T}_2$, and the correlation between the train data and test data set is small.
To go from \cref{eq:show2} to  \cref{eq:show3}, we use the following argument.
First, note $\alpha_m \leq \phi_m$ by \cref{eq:mixing relationships}. 
In addition, from the definition of $\alpha$-mixing and its moment inequality, for any bounded function $f(x)$ with a first moment, based on \citet[Theorem 14.2]{DavidsonJamesE.H1994Slta}, we have 
\begin{align*}
    \|\E[f(s_t,a_t,s_{t+1},r_t)\mid s_0,a_0,s_1,r_0]-\E[f(s_t,a_t,s_{t+1},r_t)]\|_1\leq 6\|f(s_t,a_t,s_{t+1},r_t)\|_{1}. 
\end{align*}
Note that since $\alpha$-mixing is time-reversible \citep[Page 209]{DavidsonJamesE.H1994Slta}, the following also holds:
\begin{align*}
    \|\E[f(s_0,a_0,s_{1},r_1)\mid s_t,a_t,s_{t+1},r_t]-\E[f(s_0,a_0,s_{1},r_1)]\|_1\leq 6\|f(s_0,a_0,s_{1},r_1)\|_{1}. 
\end{align*}
By applying this moment inequality to \cref{eq:show2} and noting $\psi$ is a bounded function we have
\begin{align*}
    &|\E[\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]\mid \Tcal_2]-\E[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q) |\hat w^{[2]},\hat q^{[2]}]|\\
    &= |\frac{1}{T_0}\sum_{i\in T_0}\int \{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)\} p(z_i\mid \Tcal_2)\mathrm{d}(z_i)
    -\int \braces{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)} p(z_i)\mathrm{d}(z_i) |\\
    &\leq\frac{1}{T_0}\sum_{i\in T_0}|\int \{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)\} p(z_i\mid \Tcal_2)\mathrm{d}(z_i) -\int \braces{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)} p(z_i)\mathrm{d}(z_i) |\\
    &\leq 6 \int |\braces{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)}| p(z_i)\mathrm{d}(z_i) \tag{$\alpha$-mixing moment inequality}\\
    &= 6\E[ |\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q) | \mid \hat w^{[2]},\hat q^{[2]}]=\op(1).  
\end{align*}
Then, 
\begin{align*}
    \E[\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]\mid \Tcal_2]=\E[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q) |\hat w^{[2]},\hat q^{[2]}]+\op(1). 
\end{align*}

Besides, the conditional variance is 
\begin{align}
&\mathrm{var}[\sqrt{T_0}\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]|\mathcal{T}_2] \leq \mathrm{E}[T_0\{\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]\}^2|\mathcal{T}_2]  \nonumber \\
&\leq \frac{1}{T_0}\sum_{i,j\in \ct_0}\int | \{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)\}\{\psi(z_j:\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_j;w,q)\}  p(z_i,z_j\mid \Tcal_2)\mathrm{d}(z_i,z_j) |   \label{eq:var2} \\
&=\frac{1}{T_0}\sum_{i,j\in \ct_0}\int | \{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)\}\{\psi(z_j:\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_j;w,q)\}  p(z_i,z_j)\mathrm{d}(z_i,z_j) |+\op(1)  \label{eq:var5} \\
&=\frac{1}{T_0}\left[\sum_{i=0}^{T_0} \max\{\Op((\kappa^w_N)^2),\Op((\kappa^q_N)^2)\}+2\sum_{i<j}^{T_0}\rho_{\|i-j\|} \max\{\Op((\kappa^w_N)^2),\Op((\kappa^q_N)^2)\}\right]+\smallo_p(1)  \label{eq:var3}\\
&=\smallo_p(1). \label{eq:var4}
\end{align}
Here, we used a $\alpha$-mixing condition and its moment inequality from \eqref{eq:var2} to \eqref{eq:var5}. Then, we used a $\rho$-mixing condition based on $\rho_t\leq 2\sqrt{\phi_t}=2/t^{1+\epsilon}$ (see \cref{eq:mixing relationships}) from \eqref{eq:var3} to \eqref{eq:var4}. 

Finally, based on the obtained conditional mean and conditional variance, from Chebyshev's inequality, the rest of the proof is concluded. 
\end{myproof}

\paragraph{\textbf{Second part }}
We prove 
\begin{align*}
\rE[\P_{\ct_0}[\psi(s,a,r,s';\hat{w}^{[2]},\hat{q}^{[2]})]\mid \hat{w}^{[2]},\hat{q}^{[2]}]-\rE[\psi(s,a,r,s';w,q)] = \op(T^{-1/2}).
\end{align*}
Note from \citet[Theorem 14.2]{DavidsonJamesE.H1994Slta}, 
\begin{align*}
    \|\E[f(s_0,a_0,s_{1},r_1)\mid s_t,a_t,s_{t+1},r_t]-\E[f(s_0,a_0,s_{1},r_1)]\|_1\leq 6\alpha^{1/2}_{T_0}\|f(s_0,a_0,s_{1},r_1)\|_{2}. 
\end{align*}
Then, 
\begin{align*}
    &|\E[\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]\mid \Tcal_2]-\E[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q) |\hat w^{[2]},\hat q^{[2]}]|\\
    &=\left|\E\left[\frac{1}{T_0}\sum_{i\in T_0}\int \{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)\} p(z_i\mid \Tcal_2)\mathrm{d}(z_i) -\int \braces{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)} p(z_i)\mathrm{d}(z_i)\right] \right|\\
    &\leq\frac{1}{T_0}\sum_{i\in T_0}\E[|\int \{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)\} p(z_i\mid \Tcal_2)\mathrm{d}(z_i) -\int \braces{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)} p(z_i)\mathrm{d}(z_i) |] \\
    &\leq 6\int |\braces{\psi(z_i;\hat{w}^{[2]},\hat{q}^{[2]})-\psi(z_i;w,q)}| p(z_i)\mathrm{d}(z_i) \tag{$\alpha$-mixing moment inequality}\\
    &= 6\alpha^{1/2}_{T_0}\E[ |\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q) |^2 \mid \hat w^{[2]},\hat q^{[2]}]=\op(1/\sqrt{T_0}) \tag{$\alpha_{T_0}\leq \phi_{T_0}$}.  
\end{align*}
To sum up, we have 
\begin{align}\label{eq:key_double}
    \E[\P_{\ct_0}[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q)]\mid \Tcal_2]=\E[\psi(\hat{w}^{[2]},\hat{q}^{[2]})-\psi(w,q) |\hat w^{[2]},\hat q^{[2]}]+\op(T^{-1/2}_0). 
\end{align}
Using this above, we have 
\begin{align}
&\sqrt{T}\rE[\P_{\ct_0}[\psi(s,a,r,s';\hat{w}^{[2]},\hat{q}^{[2]})]\mid \hat{w}^{[2]},\hat{q}^{[2]}] \nonumber \\
&=\sqrt{T}\rE[\rE[\P_{\ct_0}[\psi(s,a,r,s';\hat{w}^{[2]},\hat{q}^{[2]})] \mid \hat{w}^{[2]},\hat{q}^{[2]},\ct_2]\mid \hat{w}^{[2]},\hat{q}^{[2]}] \nonumber \\
&=\sqrt{T}\rE[\rE[\P_{\ct_0}[\psi(s,a,r,s';\hat{w}^{[2]},\hat{q}^{[2]})] \mid \ct_2]\mid \hat{w}^{[2]},\hat{q}^{[2]}] \nonumber\\
&=\sqrt{T}\rE[\rE[\P_{\ct_0}[\psi(s,a,r,s';\hat{w}^{[2]},\hat{q}^{[2]})]\mid \hat{w}^{[2]},\hat{q}^{[2]}]\mid \hat{w}^{[2]},\hat{q}^{[2]}]+\op(1) \tag{Use \cref{eq:key_double} } \\
&=\sqrt{T}\rE[\psi(s,a,r,s';\hat{w}^{[2]},\hat{q}^{[2]}) \mid \hat{w}^{[2]},\hat{q}^{[2]}]+\op(1) \nonumber  \\
&=\sqrt{T}\rE[\psi(s,a,r,s';w,q)]+\op(1).  \tag{The same as the proof of \cref{thm:m3_eff_cro}}
\end{align}
\paragraph{\textbf{Summary}}

Combining,  we have
\begin{align*}
    \sqrt{T}(\hat{\rho}_{\mathrm{DRL(\cm_3)}}-\rho^{\epol})=\mathbb{G}_{T}\psi(w,q)+\op(1). 
\end{align*}
The statement is concluded as in \cref{thm:ideal_m3}. 

\end{myproof}





\begin{myproof}[Proof of \cref{thm:m3_eff}]
For the ease of notation we assume $N=1$. The extension to general $N$ is straightforward. We use the same shorthand as in the proofs of \cref{thm:m3_eff_cro,thm:m3_eff_cro2}.

We have the following decomposition:
\begin{align}\label{eq:m3_eff_all}
    \sqrt{T}(\hat{\rho}_{\mathrm{DRL(\cm_3)}}-\rho^{\epol})&=\bG_{T}\psi(\hat{w},\hat{q})-\bG_{T}\psi(w,q)+\bG_{T}\psi(w,q)+\sqrt{T}(\rE[\psi(\hat{w},\hat{q})|\hat{w},\hat{q}]-\rho^{\epol}).
\end{align}

We again analyze each term.

\paragraph*{\textbf{First term}: $\bG_{T}\psi(\hat{w},\hat{q})-\bG_{T}\psi(w,q)=\op(1)$.}

From Theorem 11.24 of \citet{KosorokMichaelR2008ItEP} based on our assumptions, $\mathbb{G}_{T}\stackrel{d}{\rightarrow} \bh$ in $L^{\infty}(p_b)$, where $\bh$ is a tight mean zero Gaussian process with some covariance. By (\ref{thm:m3_eff}d), we have
$\|\psi(\hat{w},\hat{q})-\psi(w,q)\|_2=\op(1)$. Then by Lemma 18.5 of \citet{VaartA.W.vander1998As}, the statement is concluded.

\paragraph*{\textbf{Second term}: $\sqrt{T}(\rE[\psi(\hat{w},\hat{q})|\hat{w},\hat{q}]-\rho^{\epol})=\op(1).$}

The derivation is done as in the proof of \cref{thm:m3_eff_cro}. 

\paragraph*{\textbf{Summary}}
Combining,  we have
\begin{align*}
    \sqrt{T}(\hat{\rho}_{\mathrm{DRL(\cm_3)}}-\rho^{\epol})=\mathbb{G}_{T}\psi(w,q)+\op(1). 
\end{align*}
The statement is concluded as in \cref{thm:ideal_m3}. 
\end{myproof}}


{\newedit 

\begin{myproof}[Proof of \cref{thm:variance est}]
We provide the proof of cross-fitting version. The adaptive version is similarly proved. 
The estimator is given by 
\begin{align*}
\frac{n_0}{n}\P_{\Dcal_0}\psi^2_{eff}(\hat w^{[1]},\hat q^{[1]})+\frac{n_1}{n}\P_{\Dcal_1}\psi^2_{eff}(\hat w^{[0]},\hat q^{[0]}) 
\end{align*}
where $\P_{\Dcal_0}$ is a sample average over a set of samples in one fold, and  $\P_{\Dcal_1}$ is a sample average over a set of samples in another fold. Then, we have 
\begin{align}
 (\P_{\dm_0}\psi^2_{eff}(\hat w^{[1]},\hat q^{[1]})-\E[\psi^2_{eff}(w, q) ])&= \P_{\dm_0}[\psi^2_{eff}(\hat w^{[1]},\hat q^{[1]})-\psi^2_{eff}(w, q)]
    \label{eq:term3_drl_var}
    \\
    &+\sqrt{n/n_0}\bG_{n_0}[\psi^2_{eff}(w, q)]    \label{eq:term3_dr2_var}
    \\
    &+(\rE[\psi^2_{eff}(\hat w^{[1]},\hat q^{[1]})\mid \hat w^{[1]},\hat q^{[1]} ]-\E[\psi^2_{eff}(w, q) ] ).    \label{eq:term3_dr3_var}
\end{align}

We analyze each term. Here, we have 
\begin{align*}
|\psi^2_{eff}(\hat{w},\hat{q})-\psi^2_{eff}(w,q)|&=|\hat w^2\{r-\hat q(s,a)+\gamma \hat v(s')\}^2- w^2\{r- q(s,a)+\gamma v(s')\}^2|\\
&\lesssim \max\{|\hat w-w|,|\hat q-q|,|\hat v-v|\}
\end{align*}
for some constant $C$. 

\paragraph{\bf{Term \eqref{eq:term3_drl_var} is $\bigO_p(1/\sqrt{n})$ }}

The conditional mean given $\Dcal_1$ is $0$. The conditional variance given $\Dcal_1$ is  $\bigO_p(1/n)$. The rest of the argument is the same as the proof of \cref{thm:m3_inf}. 

\paragraph{\bf{Term \eqref{eq:term3_dr2_var} is $\bigO_p(1/\sqrt{n})$ }}

This is obvious. 

\paragraph{\bf{Term \eqref{eq:term3_dr3_var} is $\op(1)$ }}

\begin{align*}
    |\E[\psi^2_{eff}(\hat{w},\hat{q})-\psi^2_{eff}(w,q)\mid \Dcal_1]|&\leq C\max\{\|\hat w-w\|_2,\|\hat q-q\|_2,\|\hat v-v\|_2\}= \op(1).  
 \end{align*}

\end{myproof}
}


{\newedit 
\begin{myproof}[Proof of \cref{lem:ratio-estimation}]
Define 
\begin{align*}
    \delta(g,s')=\gamma \int p(s'|s)g(s)\mathrm{d}\lambda(s)-g(s')+(1-\gamma)p^{(0)}_{\epol}(s'),
\end{align*}
where $g(s)$ is any function and $p(s'|s)$ is a marginal distribution of $p(s'|s,a)\epol(a|s)$. Then, 
\begin{align*}
&L(w,f_w)\\
&= \rE_{p_b}[\{\gamma w(s)\eta(s,a)f_{w}(s')-w(s)f_{w}(s)\}]+(1-\gamma)\rE_{p_{\epol}^{(0)}}[f_{w}(s)] \\
    &= \rE_{p^{(\infty)}_{e,\gamma}}[(p^{(\infty)}_{e,\gamma}(s)/p_{b}(s))^{-1}\gamma w(s)\eta(s,a)f_{w}(s')]-\rE_{p^{(\infty)}_{e,\gamma}}[(p^{(\infty)}_{e,\gamma}(s)/p_{b}(s))^{-1} w(s)f_{w}(s)] \\
    &+(1-\gamma)\rE_{p_{\epol}^{(0)}}[f_{w}(s)] \\
    &= \int \delta(g,s')f_{w}(s')\mathrm{d}\lambda(s'),
\end{align*}
where we have $g(s)=p^{(\infty)}_{e,\gamma}(s)\{p^{(\infty)}_{e,\gamma}(s)/p_b(s)\}^{-1}w(s)$.

From the above, when $g(s)=p^{(\infty)}_{e,\gamma}(s)$, i.e.,  when $w(s)=p^{(\infty)}_{e,\gamma}(s)/p_{b}(s)$, $L(w,f_w)=0$. 

Conversely, $L(w,f_w)=0,\forall f_w\in L_2(S)$ means $\delta(g,s')=0$ from Riesz representation theorem. From the assumption, this means $w(s)=p^{(\infty)}_{e,\gamma}(s)/p_{b}(s)$. 
\end{myproof}
}


{\newedit 
\begin{myproof}[Proof of \cref{thm:bound_ratio}]

~
\paragraph*{\textbf{Consistency}}
We have $\hat \beta_{f_w} \stackrel{p}{\rightarrow} \beta^{*}$. We use \citet[Theorem 5.7]{VaartA.W.vander1998As}. We need to check two conditions: 
\begin{align*}
   &\sup_{\beta\in \Theta_{\beta}} |(\P_{N}-\P)[\Delta(s,a,s:\beta)] |\stackrel{p}{\rightarrow} 0,\\
   &\inf_{\|\beta-\beta_{*}\|>\epsilon}\|L(w(s:\beta,f_w))\|>0 
\end{align*}
for any $\epsilon>0$. The first condition is proved by \citet[Section 21.4]{DavidsonJamesE.H1994Slta} noting the first-order derivative of the map $\Theta_{\beta} \ni \beta \mapsto \Delta(s,a,s:\beta)$  is uniformly bounded. The second condition is proved by noting that 
\begin{align*}
    L(w(s:\beta),f_w)=0,\beta\in \Theta_{\beta}\iff \beta=\beta^{*}, 
\end{align*}
$\Theta_{\beta} \ni \beta \mapsto L(w(s:\beta)$ is continuous, and $\Theta_{\beta}$ is a compact space. 

\paragraph*{\textbf{Calculation of asymptotic variance}}

We calculate the asymptotic variance for general $f_{w}(s)$. We prove that the asymptotic MSE is given by
\begin{align}\label{eq:mainmain}
     \rE[\nabla_{\beta^{\top}}\Delta(s,a,s'; \beta)]^{-1}\rE[\Delta^{2}(s,a,s';\beta)]\{  \rE[\nabla_{\beta^{\top}}\Delta(s,a,s'; \beta)]^{-1}\}^{\top}|_{\beta^{*}}. 
\end{align}

For simplicity, we assume that $\beta$ is one-dimensional. Using mean value theorem, we have 
\begin{align}\label{eq:mainmain2}
    \sqrt{n}(\hat{\beta}_{f_w}-\beta^{*})=-\P_{n}[\nabla_{\beta^{\top}}\Delta(s,a,s'; \beta)]^{-1}|_{\beta^{\dagger}} \sqrt{n}\P_{n}[\Delta(s,a,s'; \beta)]|_{\beta^{*}},
\end{align}
where $\beta^{\dagger}$ is a value between $\hat{\beta}$ and $\beta^{*}$. The first term in right hand side of \eqref{eq:mainmain2} has the following property: 
\begin{align}
\label{eq:uni}
    \P_{n}[\nabla_{\beta^{\top}}\Delta(s,a,s'; \beta)]|_{\beta^{\dagger}}\stackrel{p}{\rightarrow} \rE[\nabla_{\beta^{\top}}\Delta(s,a,s'; \beta)]|_{\beta^{*}}.
\end{align}
This is proved by an uniform convergence condition from the fact the second-order derivative of the map $\Theta_{\beta}\ni \beta\mapsto \Delta(s,a,s';\beta)$ is uniformly bounded, and $\beta^{\dagger} \stackrel{p}{\rightarrow} \beta^{*}$.

Next, we calculate the second term in right hand size of \eqref{eq:mainmain2}. By CLT, we have 
\begin{align*}
    \sqrt{n}\P_{n}[\Delta(s,a,s'; \beta)]|_{\beta^{*}}\stackrel{d}{\rightarrow}\mathcal{N}(0,\var[\Delta(s,a,s'; \beta)]). 
\end{align*}

Finally, from Slutsky's theorem the asymptotic variance is 
\begin{align*}
   \rE[\nabla_{\beta^{\top}}\Delta(s,a,s'; \beta)]^{-1}\var[\Delta(s,a,s'; \beta)]\{\rE[\nabla_{\beta^{\top}}\Delta(s,a,s'; \beta)]^{\top}\}^{-1}|_{\beta^{*}}. 
\end{align*}

\end{myproof}
}

{\newedit
\begin{myproof}[Proof of \cref{thm:bound_ratio2}]

\begin{align*}
    \sqrt{n}(\hat{\rho}_{\mathrm{EIS}}-\rho^{\pi_e})&=  \bG_n[w(s;\hat{\beta}_{f_w})\eta(s,a)r]- \bG_n[w(s)\eta(s,a)r] \\ 
     &+\bG_n[w(s)\eta(s,a)r] + \\
     &+\sqrt{n}(\rE[w(s;\hat{\beta}_{f_w})\eta(s,a)r|\hat{\beta}_{f_w}]-\rho^{\pi_e}). 
\end{align*}
Here, from the standard argument, 
\begin{align*}
    &\sqrt{n}(\rE[w(s;\hat{\beta}_{f_w})\eta(s,a)r]-\rho^{\pi_e}) \\
    &=\sqrt{n}(\rE[w(s;\hat{\beta}_{f_w})\eta(s,a)r]-\rE[w(s;\beta^{*})\eta(s,a)r]) \\
     &=\sqrt{n}\{\rE[\nabla w(s;\beta^{*})\eta(s,a)r]|_{\beta^{*}}(\hat{\beta}_{f_w}- \beta^{*})+0.5(\hat{\beta}_{f_w}- \beta^{*})^{\top}\E[  \nabla_{\beta\beta^{\top}}\nabla w(s;\beta)\eta(s,a)r]|_{\beta^{\dagger}}(\hat{\beta}_{f_w}- \beta^{*})\} \tag{Taylor expansion} \\
    &=\rE[\nabla_{\beta^{\top}}w(s;\beta)\eta(s,a)r]\rE[\nabla_{\beta^{\top}}\Delta(s,a,s';\beta)]^{-1} \bG_n[\Delta(s,a,s';\beta)]|_{\beta^{*}}+\op(1). 
\end{align*}

Combining all together, we have
\begin{align*}
     \sqrt{n}(\hat{\rho}_{\mathrm{EIS}}-\rho^{\pi_e})= \bG_n[w(s;\beta)\eta(s,a)r+\rE[\nabla_{\beta^{\top}}w(s;\beta)\eta(s,a)r]\rE[\nabla_{\beta^{\top}}\Delta(s,a,s';\beta)]^{-1} \Delta(s,a,s';\beta)]|_{\beta^{*}}+\op(1). 
\end{align*}

\end{myproof}
}

{\newedit 
\begin{myproof}[Proof of \cref{thm:bound_q2,thm:bound_q2b}]
The proof is almost the same as the proof of \cref{thm:bound_ratio}. First, the asymptotic variance of $\hat \beta_{f_q}$ is 
\begin{align*}
    \E[f_q(s,a)\nabla_{\beta^{\top}}e_q(s,a,r,s';\beta)]^{-1}\E[f_q(s,a)f^{\top}_q(s,a)e^2_q(s,a,r,s';\beta) ]    \E[\nabla_{\beta}e_q(s,a,r,s';\beta)f^{\top}_q(s,a)]^{-1}|_{\beta^{*}} 
\end{align*}
This is equal to 
\begin{align*}
    \E[f_q(s,a)\nabla_{\beta^{\top}}m_q(s,a:\beta)]^{-1}\E[f_q(s,a)f^{\top}_q(s,a)v_q(s,a)]    \E[\nabla_{\beta}m_q(s,a:\beta)f^{\top}_q(s,a)]^{-1}|_{\beta^{*}} 
\end{align*}
Then, from \citet{matrix}, the lower bound is 
\begin{align*}
    \E[\nabla_{\beta}m(s,a;\beta)v^{-1}_q(s,a;\beta)\nabla_{\beta^{\top}}m(s,a;\beta)]|_{\beta^{*}}. 
\end{align*}
The asymptotic variance of the direct method is 
\begin{align*}
(1-\gamma)^2\E_{d_0}[\nabla_{\beta^{\top}} q(s,\epol)]  \E\left[ \frac{\otimes \{ \nabla_{\beta} \E[\gamma q(s',\pi;\beta)- q(s,a;\beta)|s,a]\}}{\mathrm{var}[r+\gamma q(s',\epol)|s,a] } \right]^{-1} \E_{d_0}[\nabla_{\beta} q(s,\epol)] .
\end{align*}
\end{myproof}

\begin{myproof}[Proof of \cref{eq:relation}]

Recall that the asymptotic variance of the direct method is 
\begin{align}\label{eq:variance}
(1-\gamma)^2\E_{d_0}[\nabla_{\beta^{\top}} q(s,\epol)]  \E\left[ \frac{\otimes \{ \nabla_{\beta} \E[\gamma q(s',\pi;\beta)- q(s,a;\beta)|s,a]\}}{\mathrm{var}[r+\gamma q(s',\epol)|s,a] } \right]^{-1} \E_{d_0}[\nabla_{\beta} q(s,\epol)] .
\end{align}
In addition, we have 
\begin{align*}
    (1-\gamma)\E_{d_0}[q(s_0,\epol)]=\E[-\gamma w(s,a)q(s',\epol)+w(s,a)q(s,a)]. 
\end{align*}
By differentiating this equation,  
\begin{align*}
    (1-\gamma)\nabla_{\beta} \E_{d_0}[q(s,\epol)]= \E[w(s,a)\nabla_{\beta}\E[-\gamma q(s',\epol)+q(s,a)|s,a]]. 
\end{align*}
According to CS-inequality, this immediately means that \eqref{eq:variance} is smaller than the efficient bound under the nonparametric model: 
\begin{align*}
    \E[w(s,a)^2\mathrm{var}[r+\gamma q(s',\epol)|s,a]]. 
\end{align*}
\end{myproof}
}

==> support.tex <==
{\blockedit 
\begin{myproof}[Proof of \cref{thm:db_m3}]
We provide the proof the cross-fitting version. The estimator is given by 
\begin{align*}
\frac{n_0}{n}\P_{\Dcal_0}\psi(\hat w^{[1]},\hat q^{[1]})+\frac{n_1}{n}\P_{\Dcal_1}\psi(\hat w^{[0]},\hat q^{[0]}) 
\end{align*}
where $\P_{\Dcal_0}$ is a sample average over a set of samples in one fold, and  $\P_{\Dcal_1}$ is a sample average over a set of samples in another fold. Then, we have 
\begin{align}
  \P_{\dm_0}\psi(\hat w^{[1]},\hat q^{[1]})&= \sqrt{1/n_0}\bG_{n_0}[\psi(\hat w^{[1]},\hat q^{[1]})-\psi(w^{\dagger}, q^{\dagger})]
    \label{eq:term3_drl}
    \\
    &+\rE[\psi(\hat w^{[1]},\hat q^{[1]})\mid \hat w^{[1]},\hat q^{[1]} ]-\rE[\psi( w^{\dagger}, q^{\dagger})]   \label{eq:term3_dr3} \\ 
    &+  \P_{\dm_0}\psi( w^{\dagger}, q^{\dagger}). 
\end{align}
Then, we have 
\begin{align*}
\rE[\psi(\hat{w},\hat{q})|\hat{w},\hat{q}]&=\rE[\{\hat{w}(s)-w^{\dagger}(s)\}\eta(s,a)\{r-q^{\dagger}(s,a)+\gamma v^{\dagger}(s')\}]+ \\
 &+\rE[w^{\dagger}(s)\eta(s,a)\{q^{\dagger}(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v^{\dagger}(s')\}]+(1-\gamma)\rE_{p^{[0]}_{e}}[v'(s)-v^{\dagger}(s)] \\
 &+\rE[\{\hat{w}(s)-w^{\dagger}(s)\}\eta(s,a)\{q^{\dagger}(s,a)-\hat{q}(s,a)+\gamma \hat{v}(s')-\gamma v^{\dagger}(s')\}] \\
 &+\rE[\{\hat{v}(s')-v^{\dagger}(s')-\hat{q}(s,a)+q^{\dagger}(s,a)\}|\hat{w},\hat{q}]\\
&+\rE[\psi(w^{\dagger},q^{\dagger})|\hat{w},\hat{q}] \\
&=\mathcal{O}(\| \hat{w}(s)-w^{\dagger}(s)\|_2,\|\hat{q}(s,a)-q^{\dagger}(s,a)\|_2,\|\hat{v}(s')-v^{\dagger}(s') \|_{2})+\rE[\psi(w^{\dagger},q^{\dagger})] \\
&=\op(1)+\rE[\psi(w^{\dagger},q^{\dagger})].
\end{align*}
Thus, the term \eqref{eq:term3_dr3} is $\op(1)$. Thus, the remaining part is proving when at least one model is well-specified, the term $\P_{\dm_0}\psi( w^{\dagger}, q^{\dagger})$ is consistent. 

\paragraph*{\bf{$q$-model is well-specified .}}

Consider the case where $q^{\dagger}(s,a)=q(s,a)$;
\begin{align*}
    &\rE[\psi(w^{\dagger},q^{\dagger})]=\rE[(1-\gamma)\rE_{p^{[0]}_{e}}[v(s)]+w^{\dagger}(s)\eta(s,a)\{r+\gamma v(s')-q(s,a)\}] \\
    &= (1-\gamma)\rE_{p^{(0)}_{e}}[v(s)]=\rho^{\epol}. 
\end{align*}
This implies when the q-model is consistent, the estimator $\hat{\rho}_{\mathrm{DRL(\cm_3)}}$ is also consistent. 

\paragraph*{\bf{$w$-model is well-specified.}}

Consider the case where $w^{\dagger}(s)=w(s)$;
\begin{align}
    \rE[\psi(w^{\dagger},q^{\dagger})]&=\rE[(1-\gamma)\rE_{p^{[0]}_{e}}[v^{\dagger}(s)]+w(s)\eta(s,a)\{r+\gamma v^{\dagger}(s')-q^{\dagger}(s,a)\}] \nonumber\\
    &=(1-\gamma)\rE_{p^{[0]}_{e}}[v^{\dagger}(s)]+\rE[w(s)\eta(s,a)r]+\rE[w(s)\eta(s,a)\gamma v^{\dagger}(s')] \label{eq:db1}\\
    &-\rE[w(s)\eta(s,a) q^{\dagger}(s,a)] \nonumber \\ 
    &=\rE[w(s)\eta(s,a)r]+\rE[w(s) v^{\dagger}(s)]-\rE[w(s)\eta(s,a) q^{\dagger}(s,a)] \label{eq:db2}\\ 
    &=\rE[w(s)\eta(s,a)r]=\rho^{\epol}.\label{eq:db3}
\end{align}
From \eqref{eq:db1} to \eqref{eq:db2}, we use a result 
\begin{align*}
    (1-\gamma)\rE_{p^{(0)}_{e}}[v^{\dagger}(s)]+\rE[w(s)\eta(s,a)\gamma v^{\dagger}(s')]=\rE[w(s) v^{\dagger}(s)]
\end{align*}
from \cref{lem:ratio-estimation}. From \eqref{eq:db2} to \eqref{eq:db3}, we use a result 
\begin{align*}
    \rE[w(s)\eta(s,a) q^{\dagger}(s,a)]= \rE[w(s)\rE[\eta(s,a) q^{\dagger}(s,a)|s]]=\rE[w(s)v^{\dagger}(s)]. 
\end{align*}
This implies when the ratio model is correct, the estimator $\hat{\rho}_{\mathrm{DRL(\cm_3)}}$ is also consistent. 


\end{myproof}
}

